An Ode to an ODE

We present a new paradigm for Neural ODE algorithms, called ODEtoODE, where time-dependent parameters of the main flow evolve according to a matrix flow on the orthogonal group O(d). This nested system of two flows, where the parameter-flow is constrained to lie on the compact manifold, provides stability and effectiveness of training and provably solves the gradient vanishing-explosion problem which is intrinsically related to training deep neural network architectures such as Neural ODEs. Consequently, it leads to better downstream models, as we show on the example of training reinforcement learning policies with evolution strategies, and in the supervised learning setting, by comparing with previous SOTA baselines. We provide strong convergence results for our proposed mechanism that are independent of the depth of the network, supporting our empirical studies. Our results show an intriguing connection between the theory of deep neural networks and the field of matrix flows on compact manifolds.

==> gradient_explosion_vanishing_calculations.tex <==
resembles residual blocks in ResNets \cite{chen2018neural} establishes the simple, yet profound connection between the worlds of deep learning and differential equations \cite{haber2017stable}. The evolution of an initial condition $\mathbf{x}_0 \in {\mathbb{R}^n}$ from $t_0$ to $t$ is given by the integral expression,
$$
\mathbf{x}_t(\theta) = \mathbf{x}_0 + \int_{t_0}^t f(\mathbf{x}(s), s, \theta) ds . \label{eq:IVP_ODE}
$$ The corresponding flow operator defined by, $$\phi_t(\mathbf{x}_0; \theta) = \mathbf{x}_t(\theta),$$ is a parametric map ${\mathbb{R}^d} \mapsto {\mathbb{R}^d}$. As such, it provides a hypothesis space for function estimation in machine learning, and may be viewed as the continuous limit of ResNet-like architectures \cite{he2016deep}. 

Reversible deep neural architecture schemes enable activations to be re-derived from those of a subsequent layer, removing the need to store them in memory \cite{gomez2017reversible}. For a Neural ODE, by construction a reversible map, loss function gradients can be computed via the adjoint sensitivity method with constant memory cost independent of depth. This decoupling of depth and memory has major implications for applications involving large inputs such as video, graphs, or 3D data \cite{davis2020time}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Stable Nonautonomous Neural ODE systems}

Consider an ordinary differential equation (ODE) defined as:
\begin{equation}
\label{ode}
\frac{d\mathbf{x}(t)}{dt} = f_{\theta}(\mathbf{x}_{t},t),    
\end{equation}
with initial condition $\mathbf{x}(0) = \mathbf{x}_{0} \in \mathbb{R}^{d}$ and where $f_{\theta}:\mathbb{R}^{d} \times \mathbb{R} \rightarrow \mathbb{R}^{d}$ for $\theta \in \mathbb{R}^{l}$. Flows that are solutions to ODEs from Equation \ref{ode} can naturally be regarded as continuous generalizations of discrete \mathrm{ResNet} architectures of the form:
\begin{equation}
\mathbf{x}_{i+1} = \mathbf{x}_{i} + \sigma(\mathbf{W}_{i}\mathbf{x}_{i} + \mathbf{b}_{i}),    
\end{equation}
for matrices $\mathbf{W}_{1},...,\mathbf{W}_{L} \in \mathbb{R}^{d \times d}$, bias vectors $\mathbf{b}_{1},...,\mathbf{b}_{L} \in \mathbb{R}^{d}$ and function $\sigma: \mathbb{R} \rightarrow \mathbb{R}$.

Considering \mathrb{ResNet}s through the lens of ODEs reveals several advantages, including: \textbf{(1)} it provides means to define deep $\mathrm{ResNet}$ architectures encoded by a compact sets of parameters (independent of the number of hidden layers $L$); \textbf{(2)} it gives rise to several new variants of computational schemes corresponding to different integrators for flows that are solutions of Equation \ref{ode}. % and more.

Standard neural ODEs, where $f_{\theta}$ is a neural network parameterized only by $\theta$, and not taking as input time $t$, correspond to autonomous systems with very limited expressiveness. Appending time $t$ as an additional input dimension helps, but the capacity of the system is still limited.
Another approach is to consider computational systems defined by ODEs of the form :
\begin{equation}
\label{ode_sigma}
\frac{d\mathbf{x}(t)}{dt} = \sigma(\mathbf{W}^{\theta}(t)\mathbf{x}_{t} + \mathbf{b}(t)),   
\end{equation}
where $\mathbf{W}^{\theta}(t):\mathbb{R} \rightarrow \mathbb{R}^{d \times d}$ is a matrix-valued function parameterized by $\theta \in \mathbb{R}^{l}$. Several classes of functions $\mathbf{W}^{\theta}(t)$ have been proposed such as those based on  trigonometric polynomials:
\begin{equation}
\mathtbf{W}^{\theta}(t)[i,j] = \sum_{k=0}^{d} a^{i,j}_{k}\sin^{k}(t) +   
\sum_{k=0}^{d} b^{i,j}_{k}\cos^{k}(t),
\end{equation}
where $\theta=[a^{i,j}_{k},b^{i,j}_{k}]^{i,j \in \{0,...,d-1\}}_{k=0,1,...,d}$ and $d$ is a hyperparameter controlling the capacity of the model.

Neural ODEs are deep computational systems and thus can suffer from the gradient vanishing/explosion problem. In particular, all previously described neural ODEs are characterized by vanishing/exploding gradients and in turn, slow training.

In this work we propose nonautonomous neural ODE systems with \textbf{provably} stable gradients. 
To do that, we encode functions $W^{\theta}(t)$ via matrix-flows on the orthogonal group $\mathcal{O}(d)$, where $\theta \in \mathbb{R}^{l}$ are the parameters of the flow. 

From the computational point of view, inference in such systems involves  computing simultaneously two flows: matrix-flow $\mathcal{F}_{\mathrm{matrix}}$ on $\mathcal{O}(d)$ and the main flow $\mathcal{F}_{\mathrm{main}}$ on $\mathbb{R}^{d}$ defined by $\mathcal{F}_{\mathrm{matrix}}$.

\subsection{Designing Stable Neural ODEs}

To design Neural ODEs with stable gradients, we first discretize Equation \ref{ode_sigma} using the standard Euler's formula to get:
\begin{equation}
\mathbf{x}_{\frac{i+1}{N}} = \mathbf{x}_{\frac{i}{N}} + \frac{1}{N} \sigma \left(\mathbf{W}^{\theta} \left(\frac{i}{N} \right)\mathbf{x}_{\frac{i}{N}}+\mathbf{b}_{\frac{i}{N}} \right),    
\end{equation}

where $i=0,1,.,,,N-1$ and $N \in \mathbb{N}_{+}$ is fixed. We assume that integration is conducted on the interval $[0,1]$.
Denote: $\mathbf{a}^{N}_{i}=\mathbf{x}_{\frac{i}{N}}$, $\mathbf{c}^{N}_{i}=\mathbf{b}_{\frac{i}{N}}$, $\mathbf{V}^{N}_{i}=\mathbf{W}^{\theta}(\frac{i}{N})$ and
$\mathbf{z}^{N}_{i+1} = \mathbf{V}^{N,\theta}_{i+1}\mathbf{a}^{N}_{i}+\mathbf{c}^{N}_{i+1}$.
We obtain the following discrete dynamical system:
\begin{equation}
\label{recurs}
\mathbf{a}^{N}_{i+1} = \mathbf{a}^{N}_{i} + \frac{1}{N}\sigma \left(\mathbf{z}^{N}_{i+1} \right) ,   
\end{equation}
for $i=0,1,...,N-1$. 


Let $\mathcal{L} = \mathcal{L}(\mathbf{x}_{1})=\mathcal{L}(\mathbf{a}^{N}_{N})$ by the loss function.
Our first goal is to compute $\frac{\partial L}{\partial \mathbf{a}^{N}_{i}}$ for $i=0,...,N-1$.

Using Equation \ref{recurs}, we get:
\begin{align}
\begin{split}
\frac{\partial L}{\partial \mathbf{a}^{N}_{i}} = 
\frac{\partial L}{\partial \mathbf{a}^{N}_{i+1}}
\frac{\partial \mathbf{a}^{N}_{i+1}}{\partial \mathbf{a}^{N}_{i}}=
\frac{\partial L}{\partial \mathbf{a}^{N}_{i+1}}(\mathbf{I}_{d}+\frac{1}{N}\mathrm{diag}(\sigma^{\prime}(\mathbf{z}^{N}_{i+1}))\frac{\partial \mathbf{z}^{N}_{i+1}}{\partial \mathbf{a}^{N}_{i}}) = \\
\frac{\partial L}{\partial \mathbf{a}^{N}_{i+1}}(\mathbf{I}_{d}+\frac{1}{N}\mathrm{diag}(\sigma^{\prime}(\mathbf{z}^{N}_{i+1})) \mathbf{V}^{N,\theta}_{i+1})
\end{split}
\end{align}

Therefore we conclude that:
\begin{equation}
\frac{\partial L}{\partial \mathbf{a}^{N}_{i}} = \frac{\partial L}{\partial \mathbf{a}^{N}_{N}}
\prod_{l=i+1}^{N} 
(\mathbf{I}_{d}+\frac{1}{N}\mathrm{diag}(\sigma^{\prime}(\mathbf{z}^{N}_{l})) \mathbf{V}^{N,\theta}_{l})
\end{equation}

{\color{blue} Valerii: "l" is already used as a dimension of $\theta$}

{\color{blue} Valerii: Either the order of multiplication should be reversed (if $\frac{\partial L}{\partial \mathbf{a}^{N}_{N}}$ is "horizontal"), or $\frac{\partial L}{\partial \mathbf{a}^{N}_{N}}$ should be on the right (if $\frac{\partial L}{\partial \mathbf{a}^{N}_{N}}}$ is "vertical").}

Note that if $\sigma(x) = |x|$ then 
$\mathrm{diag}(\sigma^{\prime}(\mathbf{z}^{N}_{l}))$ is a diagonal matrix with nonzero entries taken from $\{-1, +1\}$, in particular $D \in \mathcal{O}(d)$, where $\mathcal{O}(d)$ stands for the \textit{orthogonal group}.

Define: $\mathbf{G}^{N}_{l} = \mathrm{diag}(\sigma^{\prime}(\mathbf{z}^{N}_{l}))\mathbf{V}^{N,\theta}_{l}$.
Thus we have:
\begin{equation}
\frac{\partial L}{\partial \mathbf{a}^{N}_{i}} = \frac{\partial L}{\partial \mathbf{a}^{N}_{N}}
\prod_{l=i+1}^{N} 
(\mathbf{I}_{d}+\frac{1}{N}\mathbf{G}^{N}_{l})
\end{equation}

\begin{lemma}[Stable Gradients Lemma]
If $\mathbf{G}^{N}_{l} \in \mathcal{O}(d)$ for every $N,l$ then for any $\epsilon>0$ 
the following holds:
\begin{equation}
(\frac{1}{e} - \epsilon)\|\frac{\partial L}{\partial \mathbf{a}^{N}_{N}}\|_{2} \leq \|\frac{\partial L}{\partial \mathbf{a}^{N}_{i}}\|_{2} \leq e   
\|\frac{\partial L}{\partial \mathbf{a}^{N}_{N}}\|_{2}
\end{equation}
for $i=0,1,2,...,N-1$, where the first inequality is true for $N$ large enough ($N \geq N(\epsilon)$).
\end{lemma}

\begin{proof}
We have:
\begin{align}
\begin{split}
\prod_{l=i+1}^{N} 
(\mathbf{I}_{d}+\frac{1}{N}\mathbf{G}^{N}_{l}) = 
\sum_{\{l_{1},...,l_{k}\} \subseteq \{i+1,...,N\}} \frac{1}{N^{k}}  \mathbf{G}^{N}_{l_{1}} \cdot ... \cdot \mathbf{G}^{N}_{l_{k}}
\end{split}
\end{align}

Therefore we can conclude that:
\begin{align}
\begin{split}
\|\prod_{l=i+1}^{N} 
(\mathbf{I}_{d}+\frac{1}{N}\mathbf{G}^{N}_{l})\|_{2} \leq
\sum_{\{l_{1},...,l_{k}\} \subseteq \{i+1,...,N\}} \frac{1}{N^{k}}  \|\mathbf{G}^{N}_{l_{1}} \cdot ... \cdot \mathbf{G}^{N}_{l_{k}}\|_{2} \\  = \sum_{k=0}^{N-i} \frac{1}{N^{k}}{N-i \choose k} = \sum_{k=0}^{N-i}\frac{(N-i-k+1)\cdot...\cdot (N-i)}{N^{k}k!} \leq \sum_{k=0}^{N-i} \frac{1}{k!} \leq e,
\end{split}    
\end{align}
where we used the fact that $\mathcal{O}(d)$ is a group under matrix-multiplication and $\|\mathbf{G}\|_{2} = 1$ for every $\mathbf{G} \in \mathcal{O}(d)$.
That proves inequality: $\|\frac{\partial L}{\partial \mathbf{a}^{N}_{i}}\|_{2} \leq e   
\|\frac{\partial L}{\partial \mathbf{a}^{N}_{N}}\|_{2}$. 

To prove that: $\|\frac{\partial L}{\partial \mathbf{a}^{N}_{i}}\|_{2} \geq (\frac{1}{e}-\epsilon)   
\|\frac{\partial L}{\partial \mathbf{a}^{N}_{N}}\|_{2}$, for large enough $N \geq N(\epsilon)$, it suffices to observe that if $\mathbf{G} \in \mathcal{O}(d)$, then for any $\mathbf{v} \in \mathbb{R}^{d}$ we have (by triangle inequality):
\begin{equation}
\|(\mathbf{I}_{d} + \frac{1}{N}\mathbf{G})\mathbf{v}\|_{2} \geq    
\|\mathbf{v}\|_{2} - \|\frac{1}{N}\mathbf{Gv}\|_{2}=(1-\frac{1}{N})\|\mathbf{v}\|_{2}.
\end{equation}

The inequality then follows immediately from the fact that sequence: $\{a_{N}:N=1,2,3,...\}$ defined as: $a_{N}=(1-\frac{1}{N})^{N}$ has limit $e^{-1}$.

\end{proof}

==> method.tex <==
a Nested ODE structure where the function q is defined by a Gated HyperNet, defined as:

% Need to compress the below notation:
\begin{equation} \label{eq:parent_network}
z_t(\theta) = z_0 + \int_{0}^1 f(z(t), t, \theta(t)) dt \label{eq:IVP_ODE}
\end{equation}
with 
\begin{equation} \label{eq:weight_network}
\theta(t) = \theta(0) + \int_{t_0}^t q(\theta(t), \alpha) dt \label{eq:IVP_Nested}.
\end{equation}
$\mathrm{q}$ is defined by a gating mechanism $\sigma{(t)}$ that combines $d$ different potential hidden dynamics $f$ in a proportion defined by a sigmoid. This results in 

\begin{equation} \label{eq:hyper_gate}
\mathrm{q}_{t} = \sum\limits_{n=1}^d\sigma_n{(t)}f_n(\textbf{h}_{t}, \theta_t),
\end{equation}

with $\sigma_n{(t)} \in (0, 1)$ output by a neural network parameterized by weights $\alpha$. This is inspired by the gating mechanism briefly discussed in \cite{} for Continuous Normalizing Flows.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For $\mathrm{ODEtoODE}$ Linear, we define the evolution of the hidden dynamics as a Flow parameterized by matrices $\mathbf{N}$ and $\mathbf{Q}$ (see: Sec ??)

For ODEtoODELinear we use an eta of .01 as well. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[th!]
\caption{Performance Comparison}\label{table1}
\centering\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}>{\bfseries}l*{11}{r}@{}}

\toprule[1pt]
\multicolumn{18}{@{}c@{}}{}\\
\midrule[0.75pt]

Models & \textbf{Dense-1} & \textbf{Dense-10} & \textbf{NODE}& \textbf{NANODE-1} & \textbf{NANODE-10} & \textbf{HyperNet-1} & \textbf{HyperNet-10} & \textbf{ODEtoODE-1} & \textbf{ODEtoODE-10} & \textbf{ODEtoODE-L} & \\
\midrule[0.75pt]

ZigZag & 73.95 & 68.44 & 70.13 & 74.24 & 74.71 & 75.11 & 74.8 & 78.68 & \textbf{79.48} & 75.5 &  \\
Canny Edges & \textbf{61.74} & 41.36 & 52.94 & 51.39 &	49.78 &	49.29 &	49.96 &	60.77 &	59.2 &	59.42 & \\
Dotted Lines & 92.99 & 88.22	& 91.54	& 92.42	& 92.74	& 91.88 & 91.9 & \textbf{95.42} & 95.22 & 94.22 & \\
Spatter & 93.54 & 89.52	& 92.49	& 93.13	& 93.15	& 93.19	& 93.28	& \textbf{94.9}	& \textbf{94.9}	& 94.2 & \\
Stripe & 30.55 & 20.57 & 36.76	& 16.4	& 21.37	& 19.71	& 18.69	& \textbf{44.51} & 44.37	& 35.9 & \\
Translate & 25.8 & 24.82	& 27.09	& 28.97	& 29.31	& \textbf{29.42} & 29.3	& 26.82	& 26.63	& 25.27 & \\
Rotate & 82.8 & 80.38	& 82.76	& 83.19	& 83.65	& 83.5	& 83.56	& 83.9 & \textbf{84.1}	& 82.62 \\
Scale & 58.68 & 62.73	& 62.05	& 66.43	& 66.63	& 67.84	& \textbf{68.11} & 66.68 & 66.76	& 60.66 \\
Shear & 91.73 & 89.52	& 91.82	& 92.18	& 93.11	& 92.33	& 92.48	& \textbf{93.37} & 92.93	& 91.66 \\
Motion Blur & 78.16 & 67.25	& 75.18	& 76.53	& \textbf{79.22}	& 78.82	& 78.33	& 78.63	& 77.58	& 76.48 \\
Glass Blur & 91.62 & 84.89	& 87.94	& 90.18	& 91.07	& 91.3	& 91.17	& \textbf{93.91} & 93.29	& 91.86 \\
Impulse Noise  & 76.93 & 61.42 & 71.18 & 66.68 & 63.34 & 65.75 & 65.52 & \textbf{85.71} & 84.01 & 79.44 \\
Shot Noise & 96.16 & 91.63 & 94.24 & 94.97 & 94.73 & 94.76 & 94.81 & \textbf{96.91} & 96.71 & 96.24 \\
Identity & 97.55 & 95.73	& 97.61	& 97.65	& 97.69	& 97.72	& 97.54	& \textbf{97.94} & 97.88	& 97.76 \\
CIFAR10 & 52.83	& 50.53	& 51.47	& 53.24	& \textbf{54.27} & 51.85	& 52.6	& 52.99	& 53.07	& 50.74 \\

\bottomrule[2pt]
\addlinespace[3pt]
\end{tabular}}
\end{table}

% probably will put this in the appendix
\begin{table}[th!]
\caption{Additional Sweep}\label{table2}
\centering\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}>{\bfseries}l*{14}{r}@{}}

\toprule[1pt]
\multicolumn{18}{@{}c@{}}{}\\
\midrule[0.75pt]

Models & \textbf{Dense-1} & \textbf{Dense-2} & \textbf{Dense-4} & \textbf{NODE} & \textbf{NANODE-1} & \textbf{NANODE-2} & \textbf{NANODE-4} & \textbf{HyperNet-1} & \textbf{HyperNet-2} & \textbf{HyperNet-4} & \textbf{ODEtoODE-1} & \textbf{ODEtoODE-2} & \textbf{ODEtoODE-4} & \textbf{ODEODE-L} & \\
\midrule[0.75pt]

ZigZag & 74.91 & 74.85 & 74.58 &	73.64 &	72.25 &	72.72 &	73.12 &	74.96	& 74.85	& 75.13 &	79.98 &	79.34 &	79.42	& 78.11  \\
Canny Edges & 60.98 &	56.03 &	51.17 &	50.93 &	51.21 &	50.59 &	49.66	& 53.81 &	53.54 &	53.48 &	60.73 &	60.75 &	61.31 &	62.62 \\
Dotted Line	& 94.47 &	93.21 &	91.88 &	92.9 &	92 &	92.02 &	92.02 &	92.35 &	92.91 &	92.57 &	95.64 &	95.66 &	95.6 &	95.2 \\
Spatter	& 94.52	& 93.59	& 93.63 &	93.32 &	92.81 &	92.82 &	92.84 &	94.09	& 93.94	& 93.73	& 95.28	& 95.47	& 95.29	& 95.08 \\
Stripe & 29.69	& 32.73	 & 31.49 &	36.08 &	27.32 &	23.56 &	24.66 &	30.86	& 31.12 &	29.1	& 36.25	& 28.21	& 31.91 &	30.08 \\
Translate	& 25.85	& 28.35	& 27.27	& 29.13	& 29.11 &	29.24 &	28.7	& 29.85 &	29.68 &	29.87 &	25.61 &	26.1 &	26.42 &	25.96 \\
Rotate & 83.62	& 83.73 & 83.88 &	83.09 &	82.5 &	82.77 & 83.03 & 83.96	& 84.04	& 84.13 &	85.1 &	85.03 &	84.72 &	84.16 \\
Scale & 61.41	& 65.07 & 63.72 &	63.62	& 65.49	& 65.33 &	64.03	& 69.51 &	68.77	& 69.8	& 67.97	& 66.95	& 67.09 &	60.91 \\
Shear & 92.25 &	92.76 &	92.55 &	92.27 &	92.08 &	92.18 &	92.3 &	93.35	& 92.84	& 93.04	& 93.15 &	93.06 &	93.38 &	92.59 \\
Motion Blur	& 76.47 & 73.89 &	74.95 &	76.3 &	75.24	& 75.88	& 76.22	& 80.67 &	81.26 &	81.36 &	78.92 &	79.11 &	79.02 &	79.55 \\
Glass Blur & 92.5 &	89.65 &	90.29 &	89.47 &	89.5 &	89.5 &	89.8 &	93.07 &	92.67 &	92.69 &	94.46 &	94.19 &	94.3 &	93.53 \\
Impulse Noise & 80.98 & 75.03 &	72.9 &	70.63 &	68.04 &	67.72 &	67.5	& 74.63 &	74.53 &	73.31 &	84.51 &	84.21 &	83.8 &	83.11 \\
Shot Noise & 96.41 & 95.78 &	95.22 &	95.09 &	94.18  &	94.12 &	93.85 &	95.36 &	96.88 &	96.77 &	96.93 &	96.88 &	96.77 &	96.51 \\
Identity & 97.7 & 97.75 &	97.71 &	97.64 &	97.6 &	97.5 &	97.52 &	97.7	& 97.82	& 97.79 &	98.03 &	98.12 &	98.11 &	97.82 \\
CIFAR10 & 52.83 & 53.39 &	52.38 &	51.24 &	53.04 &	52.17 &	52.57 &	54.44	& 53.66	& 54.68 &	53.58 &	55.02 &	53.97 &	51.87 \\


\end{tabular}}
\end{table}
